Graphical X Splatting (GraphiXS): A Graphical Model for 4D Gaussian Splatting under Uncertainty

We propose a new framework to systematically incorporate data uncertainty in Gaussian Splatting. Being the new paradigm of neural rendering, Gaussian Splatting has been investigated in many applications, with the main effort in extending its representation, improving its optimization process, and accelerating its speed. However, one orthogonal, much needed, but under-explored area is data uncertainty. In standard 4D Gaussian Splatting, data uncertainty can manifest as view sparsity, missing frames, camera asynchronization, etc. So far, there has been little research to holistically incorporating various types of data uncertainty under a single framework. To this end, we propose Graphical X Splatting, or GraphiXS, a new probabilistic framework that considers multiple types of data uncertainty, aiming for a fundamental augmentation of the current 4D Gaussian Splatting paradigm into a probabilistic setting. GraphiXS is general and can be instantiated with a range of primitives, e.g. Gaussians, Student's-t. Furthermore, GraphiXS can be used to `upgrade' existing methods to accommodate data uncertainty. Through exhaustive evaluation and comparison, we demonstrate that GraphiXS can systematically model various uncertainties in data, outperform existing methods in many settings where data are missing or polluted in space and time, and therefore is a major generalization of the current 4D Gaussian Splatting research.

==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{blue}[TODO: #1]}}
\newcommand{\HW}[1]{\textbf{\color{red}[HW: #1]}}
\newcommand{\added}[1]{\textcolor{green!60!black}{#1}}
\newcommand{\removed}[1]{\textcolor{red!70!black}{\sout{#1}}}

\RequirePackage{times}    % Integrate Times for here
\RequirePackage{xspace}
\RequirePackage[dvipsnames]{xcolor}
\RequirePackage{graphicx}
\RequirePackage{amsmath}
\RequirePackage{booktabs}
\usepackage{bibunits}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} \def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother


\newcommand{\mat}[1]{\mathbf{#1}}


\AtEndPreamble{
    \usepackage[capitalize]{cleveref}
    \crefname{section}{Sec.}{Secs.}
    \Crefname{section}{Section}{Sections}
    \Crefname{table}{Table}{Tables}
    \crefname{table}{Tab.}{Tabs.}
}

%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

\usepackage{colortbl}
\usepackage{multirow}
\usepackage{stfloats}
\usepackage{tabularx}


\renewcommand{\dbltopfraction}{0.95} % Allow top floats to take up to 95% of the page
\renewcommand{\dblfloatpagefraction}{0.95} % Require floats to take up 95% of a page before getting their own dedicated page
\renewcommand{\textfraction}{0.05} % Allow pages to have as little as 5% text

\usepackage{enumitem}
\setlist[itemize]{noitemsep, topsep=2pt, parsep=0pt, partopsep=0pt}
\setlist[enumerate]{noitemsep, topsep=2pt, parsep=0pt, partopsep=0pt}

\setlength{\textfloatsep}{12pt}
\setlength{\floatsep}{12pt}
\setlength{\intextsep}{12pt}
\setlength{\tabcolsep}{3pt}

\setlength{\abovecaptionskip}{4pt}
\setlength{\belowcaptionskip}{0pt}

% Define colors
\definecolor{best}{HTML}{D5E8D4} %Light Green 
\definecolor{second}{HTML}{FFF2CC} % Light Yellow 

\newcommand{\colw}{0.135\textwidth}

\newcommand{\figrow}[2]{%
    \textbf{#1}\par\vspace{1pt}

    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/4dgs_iclr.jpg}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/4dgs_iclr_a.jpg}\hfill
        \includegraphics[width=0.49\linewidth]{#2/4dgs_iclr_b.jpg}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/4dgs_cvpr.jpg}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/4dgs_cvpr_a.jpg}\hfill
        \includegraphics[width=0.49\linewidth]{#2/4dgs_cvpr_b.jpg}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/ex4dgs.jpg}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/ex4dgs_a.jpg}\hfill
        \includegraphics[width=0.49\linewidth]{#2/ex4dgs_b.jpg}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/ftgs.jpg}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/ftgs_a.jpg}\hfill
        \includegraphics[width=0.49\linewidth]{#2/ftgs_b.jpg}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/graphigs.jpg}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/graphigs_a.jpg}\hfill
        \includegraphics[width=0.49\linewidth]{#2/graphigs_b.jpg}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/graphits.jpg}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/graphits_a.jpg}\hfill
        \includegraphics[width=0.49\linewidth]{#2/graphits_b.jpg}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/gt.jpg}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/gt_a.jpg}\hfill
        \includegraphics[width=0.49\linewidth]{#2/gt_b.jpg}
    \end{minipage}

    \par\vspace{1pt}
}

% ===== SPLIT LAYOUT (4 items top, 3 items bottom) =====
\newcommand{\figrowSplit}[1]{%

  \def\sw{0.24\linewidth}%
  
  % --- ROW 1: Competitors (4 items) ---
  \begin{minipage}[t]{\sw}\centering\scriptsize 4DGS-1 \cite{yang2023gs4d}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/4dgs_iclr.jpg}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/4dgs_iclr_a.jpg}\hfill
    \includegraphics[width=0.49\linewidth]{#1/4dgs_iclr_b.jpg}
  \end{minipage}\hfill
  \begin{minipage}[t]{\sw}\centering\scriptsize 4DGS-2 \cite{wu20244d}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/4dgs_cvpr.jpg}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/4dgs_cvpr_a.jpg}\hfill
    \includegraphics[width=0.49\linewidth]{#1/4dgs_cvpr_b.jpg}
  \end{minipage}\hfill
  \begin{minipage}[t]{\sw}\centering\scriptsize Ex4DGS \cite{lee2024fully}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/ex4dgs.jpg}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/ex4dgs_a.jpg}\hfill
    \includegraphics[width=0.49\linewidth]{#1/ex4dgs_b.jpg}
  \end{minipage}\hfill
  \begin{minipage}[t]{\sw}\centering\scriptsize FTGS \cite{wang2025freetimegs}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/ftgs.jpg}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/ftgs_a.jpg}\hfill
    \includegraphics[width=0.49\linewidth]{#1/ftgs_b.jpg}
  \end{minipage}
  
  \par\vspace{6pt} % Gap between top and bottom rows
  
  % --- ROW 2: Ours + GT (3 items, Centered) ---
  {\centering
  \begin{minipage}[t]{\sw}\centering\scriptsize \textbf{Ours (GraphiGS)}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/graphigs.jpg}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/graphigs_a.jpg}\hfill
    \includegraphics[width=0.49\linewidth]{#1/graphigs_b.jpg}
  \end{minipage}\hspace{2mm} % Slight gap
  \begin{minipage}[t]{\sw}\centering\scriptsize \textbf{Ours (GraphiTS)}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/graphits.jpg}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/graphits_a.jpg}\hfill
    \includegraphics[width=0.49\linewidth]{#1/graphits_b.jpg}
  \end{minipage}\hspace{2mm} % Slight gap
  \begin{minipage}[t]{\sw}\centering\scriptsize GT\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/gt.jpg}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/gt_a.jpg}\hfill
    \includegraphics[width=0.49\linewidth]{#1/gt_b.jpg}
  \end{minipage}
  \par}
}

\newcommand{\figrowCrops}[1]{%
  % Configuration
  \setlength{\tabcolsep}{1pt} % Minimal horizontal gap
  \renewcommand{\arraystretch}{0.5} % Minimal vertical gap
  
  % --- Left Block: Full Ground Truth ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    % Label in 2 lines to match the height of headers on the right
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.jpg}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: 6 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    \begin{tabular}{@{}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row: Method Names ---
      % Note: I used \parbox on the left label, so these will align nicely
      \parbox{1.6cm}{\centering 4DGS-1\\\cite{yang2023gs4d}} & 
      \parbox{1.6cm}{\centering 4DGS-2\\\cite{wu20244d}} & 
      \parbox{1.6cm}{\centering Ex4DGS\\\cite{lee2024fully}} & 
      \parbox{1.6cm}{\centering FTGS\\\cite{wang2025freetimegs}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiGS}\\\textbf{(Ours)}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiTS}\\\textbf{(Ours)}} \\[5pt]
      
      % --- Row 1: Crop A ---
      % Width 0.163 fills the 6-column space perfectly (6 * 0.163 ~ 0.98)
      \includegraphics[width=0.163\linewidth]{#1/4dgs_iclr_a.jpg} &
      \includegraphics[width=0.163\linewidth]{#1/4dgs_cvpr_a.jpg} &
      \includegraphics[width=0.163\linewidth]{#1/ex4dgs_a.jpg} &
      \includegraphics[width=0.163\linewidth]{#1/ftgs_a.jpg} &
      \includegraphics[width=0.163\linewidth]{#1/graphigs_a.jpg} &
      \includegraphics[width=0.163\linewidth]{#1/graphits_a.jpg} \\[1pt]

      % --- Row 2: Crop B ---
      \includegraphics[width=0.163\linewidth]{#1/4dgs_iclr_b.jpg} &
      \includegraphics[width=0.163\linewidth]{#1/4dgs_cvpr_b.jpg} &
      \includegraphics[width=0.163\linewidth]{#1/ex4dgs_b.jpg} &
      \includegraphics[width=0.163\linewidth]{#1/ftgs_b.jpg} &
      \includegraphics[width=0.163\linewidth]{#1/graphigs_b.jpg} &
      \includegraphics[width=0.163\linewidth]{#1/graphits_b.jpg} \\
      
    \end{tabular}
  \end{minipage}
}

\newcommand{\figrowCropsTwoRowWL}[5]{%
  % Configuration
  \setlength{\tabcolsep}{0pt} % We control spacing manually with @{\hspace{...}}
  \renewcommand{\arraystretch}{0.5} % Keep text tight
  
  % --- Internal Helpers for Vertical Centering ---
  % Wraps image in a box aligned at its vertical center
  \def\vcimg##1{\parbox[c]{0.153\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
  % Wraps label in a box aligned at its vertical center
  \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
  % --- Left Block: Full Ground Truth (Unchanged) ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    % Label in 2 lines to match the height of headers on the right
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.jpg}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: Labels + 6 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    % 7 columns: 1 label column + 6 method columns
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row: Method Names ---
      &
      \parbox{1.6cm}{\centering 4DGS-1\\\cite{yang2023gs4d}} & 
      \parbox{1.6cm}{\centering 4DGS-2\\\cite{wu20244d}} & 
      \parbox{1.6cm}{\centering Ex4DGS\\\cite{lee2024fully}} & 
      \parbox{1.6cm}{\centering FTGS\\\cite{wang2025freetimegs}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiGS}\\\textbf{(Ours)}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiTS}\\\textbf{(Ours)}} \\[5pt]
      
      % --- Row 1: Crop A ---
      \vclbl{#4} &
      \vcimg{#1/4dgs_iclr_#2_a.jpg} &
      \vcimg{#1/4dgs_cvpr_#2_a.jpg} &
      \vcimg{#1/ex4dgs_#2_a.jpg} &
      \vcimg{#1/ftgs_#2_a.jpg} &
      \vcimg{#1/graphigs_#2_a.jpg} &
      \vcimg{#1/graphits_#2_a.jpg} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 2: Crop B ---
      \vclbl{#5} &
      \vcimg{#1/4dgs_iclr_#3_a.jpg} &
      \vcimg{#1/4dgs_cvpr_#3_a.jpg} &
      \vcimg{#1/ex4dgs_#3_a.jpg} &
      \vcimg{#1/ftgs_#3_a.jpg} &
      \vcimg{#1/graphigs_#3_a.jpg} &
      \vcimg{#1/graphits_#3_a.jpg} \\
      
    \end{tabular}
  \end{minipage}
}

\newcommand{\figrowCropsThreeRowWL}[7]{%
  % Configuration
  \setlength{\tabcolsep}{0pt} % We control spacing manually with @{\hspace{...}}
  \renewcommand{\arraystretch}{0.5} % Keep text tight
  
  % --- Internal Helpers for Vertical Centering ---
  % Wraps image in a box aligned at its vertical center
  \def\vcimg##1{\parbox[c]{0.153\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
  % Wraps label in a box aligned at its vertical center
  \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
  % --- Left Block: Full Ground Truth ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.jpg}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: Labels + 6 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    % 7 columns: Label + 1pt Gap + Method + 1pt Gap + Method ...
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row ---
      &
      \parbox{1.6cm}{\centering 4DGS-1\\\cite{yang2023gs4d}} & 
      \parbox{1.6cm}{\centering 4DGS-2\\\cite{wu20244d}} & 
      \parbox{1.6cm}{\centering Ex4DGS\\\cite{lee2024fully}} & 
      \parbox{1.6cm}{\centering FTGS\\\cite{wang2025freetimegs}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiGS}\\\textbf{(Ours)}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiTS}\\\textbf{(Ours)}} \\[5pt]
      
      % --- Row 1: Crop A ---
      \vclbl{#5} &
      \vcimg{#1/4dgs_iclr_#2_a.jpg} &
      \vcimg{#1/4dgs_cvpr_#2_a.jpg} &
      \vcimg{#1/ex4dgs_#2_a.jpg} &
      \vcimg{#1/ftgs_#2_a.jpg} &
      \vcimg{#1/graphigs_#2_a.jpg} &
      \vcimg{#1/graphits_#2_a.jpg} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 2: Crop B ---
      \vclbl{#6} &
      \vcimg{#1/4dgs_iclr_#3_a.jpg} &
      \vcimg{#1/4dgs_cvpr_#3_a.jpg} &
      \vcimg{#1/ex4dgs_#3_a.jpg} &
      \vcimg{#1/ftgs_#3_a.jpg} &
      \vcimg{#1/graphigs_#3_a.jpg} &
      \vcimg{#1/graphits_#3_a.jpg} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 3: Crop C ---
      \vclbl{#7} &
      \vcimg{#1/4dgs_iclr_#4_a.jpg} &
      \vcimg{#1/4dgs_cvpr_#4_a.jpg} &
      \vcimg{#1/ex4dgs_#4_a.jpg} &
      \vcimg{#1/ftgs_#4_a.jpg} &
      \vcimg{#1/graphigs_#4_a.jpg} &
      \vcimg{#1/graphits_#4_a.jpg} \\
      
    \end{tabular}
  \end{minipage}
}

\newcommand{\figrowCropsTwoRowWLShort}[5]{%
  % Configuration
  \setlength{\tabcolsep}{0pt} % We control spacing manually with @{\hspace{...}}
  \renewcommand{\arraystretch}{0.5} % Keep text tight
  
  % --- Internal Helpers for Vertical Centering ---
  % Increased width to 0.235 to fill space with only 4 images
  \def\vcimg##1{\parbox[c]{0.21\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
  \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
  % --- Left Block: Full Ground Truth ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.jpg}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: Labels + 4 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    % 5 columns: 1 label column + 4 method columns
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row ---
      % Parbox width increased to 2.5cm to match larger image width
      &
      \parbox{2.5cm}{\centering W/O Upgrade} & 
      \parbox{2.5cm}{\centering W Upgrade} & 
      \parbox{2.5cm}{\centering W/O Upgrade} & 
      \parbox{2.5cm}{\centering W Upgrade} \\[5pt]
      
      % --- Row 1: Crop A ---
      % Uses #2 for filename suffix, #4 for Label
      \vclbl{#4} &
      \vcimg{#1/ftgs_#2_a.jpg} &
      \vcimg{#1/upgrade_#2_a.jpg} &
      \vcimg{#1/ftgs_#2_b.jpg} &
      \vcimg{#1/upgrade_#2_b.jpg} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 2: Crop B ---
      % Uses #3 for filename suffix, #5 for Label
      \vclbl{#5} &
      \vcimg{#1/ftgs_#3_a.jpg} &
      \vcimg{#1/upgrade_#3_a.jpg} &
      \vcimg{#1/ftgs_#3_b.jpg} &
      \vcimg{#1/upgrade_#3_b.jpg} \\
      
    \end{tabular}
  \end{minipage}
}

\newcommand{\figrowCropsTwoRowWLShortAbl}[5]{%
  % Configuration
  \setlength{\tabcolsep}{0pt} % We control spacing manually with @{\hspace{...}}
  \renewcommand{\arraystretch}{0.5} % Keep text tight
  
  % --- Internal Helpers for Vertical Centering ---
  % Increased width to 0.235 to fill space with only 4 images
  \def\vcimg##1{\parbox[c]{0.21\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
  \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
  % --- Left Block: Full Ground Truth ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.jpg}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: Labels + 4 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    % 5 columns: 1 label column + 4 method columns
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row ---
      % Parbox width increased to 2.5cm to match larger image width
      &
      \parbox{2.5cm}{\centering W/O Higher\\Order Dynamics} & 
      \parbox{2.5cm}{\centering W/O $P(\alpha \mid \theta, C, T)$} & 
      \parbox{2.5cm}{\centering W/O\\Stochasticity} & 
      \parbox{2.5cm}{\centering \textbf{GraphiTS (Ours)}} \\[5pt]
      
      % --- Row 1: Crop A ---
      \vclbl{#4} &
      \vcimg{#1/no_higher_#2_a.jpg} &
      \vcimg{#1/no_likeli_#2_a.jpg} &
      \vcimg{#1/deterministic_#2_a.jpg} &
      \vcimg{#1/graphits_#2_a.jpg} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 2: Crop B ---
      \vclbl{#5} &
      \vcimg{#1/no_higher_#3_a.jpg} &
      \vcimg{#1/no_likeli_#3_a.jpg} &
      \vcimg{#1/deterministic_#3_a.jpg} &
      \vcimg{#1/graphits_#3_a.jpg} \\
      
    \end{tabular}
  \end{minipage}
}
